RELEAF: An Algorithm for Learning and Exploiting Relevance

Recommender systems, medical diagnosis, network security, etc., require on-going learning and decision-making in real time. These -- and many others -- represent perfect examples of the opportunities and difficulties presented by Big Data: the available information often arrives from a variety of sources and has diverse features so that learning from all the sources may be valuable but integrating what is learned is subject to the curse of dimensionality. This paper develops and analyzes algorithms that allow efficient learning and decision-making while avoiding the curse of dimensionality. We formalize the information available to the learner/decision-maker at a particular time as a context vector which the learner should consider when taking actions. In general the context vector is very high dimensional, but in many settings, the most relevant information is embedded into only a few relevant dimensions. If these relevant dimensions were known in advance, the problem would be simple -- but they are not. Moreover, the relevant dimensions may be different for different actions. Our algorithm learns the relevant dimensions for each action, and makes decisions based in what it has learned. Formally, we build on the structure of a contextual multi-armed bandit by adding and exploiting a relevance relation. We prove a general regret bound for our algorithm whose time order depends only on the maximum number of relevant dimensions among all the actions, which in the special case where the relevance relation is single-valued (a function), reduces to $\tilde{O}(T^{2(\sqrt{2}-1)})$; in the absence of a relevance relation, the best known contextual bandit algorithms achieve regret $\tilde{O}(T^{(D+1)/(D+2)})$, where $D$ is the full dimension of the context vector.

==> OSA.tex <==
%MAY 4 REFERENCES - EXPERTS AND ACTIVE LEARNING

@article{baram2004online,
  title={Online choice of active learning algorithms},
  author={Baram, Yoram and El-Yaniv, Ran and Luz, Kobi},
  journal={The Journal of Machine Learning Research},
  volume={5},
  pages={255--291},
  year={2004},
  publisher={JMLR. org}
}

@article{angluin1988queries,
  title={Queries and concept learning},
  author={Angluin, Dana},
  journal={Machine learning},
  volume={2},
  number={4},
  pages={319--342},
  year={1988},
  publisher={Springer}
}

@article{cesa1997use,
  title={How to use expert advice},
  author={Cesa-Bianchi, Nicolo and Freund, Yoav and Haussler, David and Helmbold, David P and Schapire, Robert E and Warmuth, Manfred K},
  journal={Journal of the ACM (JACM)},
  volume={44},
  number={3},
  pages={427--485},
  year={1997},
  publisher={ACM}
}

@article{cesa2005minimizing,
  title={Minimizing regret with label efficient prediction},
  author={Cesa-Bianchi, Nicolo and Lugosi, G{\'a}bor and Stoltz, Gilles},
  journal={Information Theory, IEEE Transactions on},
  volume={51},
  number={6},
  pages={2152--2162},
  year={2005},
  publisher={IEEE}
}

@inproceedings{zolghadr2013online,
  title={Online Learning with Costly Features and Labels},
  author={Zolghadr, Navid and Bart{\'o}k, G{\'a}bor and Greiner, Russell and Gy{\"o}rgy, Andr{\'a}s and Szepesv{\'a}ri, Csaba},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1241--1249},
  year={2013}
}

@article{dekel2012selective,
  title={Selective sampling and active learning from single and multiple teachers},
  author={Dekel, Ofer and Gentile, Claudio and Sridharan, Karthik},
  journal={The Journal of Machine Learning Research},
  volume={13},
  number={1},
  pages={2655--2697},
  year={2012},
  publisher={JMLR. org}
}

%APRIL 29 REFERENCES

@inproceedings{xu2013department,
  title={Department of Electrical Engineering, University of California, Los Angeles (UCLA), USA},
  author={Xu, Jie and Tekin, Cem and van der Schaar, Mihaela},
  booktitle={Communication, Control, and Computing (Allerton), 2013 51st Annual Allerton Conference on},
  pages={512--519},
  year={2013},
  organization={IEEE}
}

@article{adiga2006high,
  title={High-throughput analysis of multispectral images of breast cancer tissue},
  author={Adiga, Umesh and Malladi, Ravi and Fernandez-Gonzalez, Rodrigo and de Solorzano, C Ortiz},
  journal={Image Processing, IEEE Transactions on},
  volume={15},
  number={8},
  pages={2259--2268},
  year={2006},
  publisher={IEEE}
}

@article{schnorrenberg1997computer,
  title={Computer-aided detection of breast cancer nuclei},
  author={Schnorrenberg, Frank and Pattichis, Constantinos S and Kyriacou, Kyriacos C and Schizas, Christos N},
  journal={Information Technology in Biomedicine, IEEE Transactions on},
  volume={1},
  number={2},
  pages={128--140},
  year={1997},
  publisher={IEEE}
}

@article{foo2010distributed,
  title={A distributed approach for optimizing cascaded classifier topologies in real-time stream mining systems},
  author={Foo, Brian and van der Schaar, Mihaela},
  journal={Image Processing, IEEE Transactions on},
  volume={19},
  number={11},
  pages={3035--3048},
  year={2010},
  publisher={IEEE}
}

@article{bouguila2006hybrid,
  title={A hybrid SEM algorithm for high-dimensional unsupervised learning using a finite generalized Dirichlet mixture},
  author={Bouguila, Nizar and Ziou, Djemel},
  journal={Image Processing, IEEE Transactions on},
  volume={15},
  number={9},
  pages={2657--2668},
  year={2006},
  publisher={IEEE}
}

@article{liu2001multiresolution,
  title={Multiresolution detection of spiculated lesions in digital mammograms},
  author={Liu, Sheng and Babbs, Charles F and Delp, Edward J},
  journal={Image Processing, IEEE Transactions on},
  volume={10},
  number={6},
  pages={874--884},
  year={2001},
  publisher={IEEE}
}

@inproceedings{kohavi1996scaling,
  title={Scaling up the accuracy of naive-Bayes classifiers: A decision-tree hybrid.},
  author={Kohavi, Ron},
  booktitle={KDD},
  pages={202--207},
  year={1996}
}

@article{schein2007active,
  title={Active learning for logistic regression: an evaluation},
  author={Schein, Andrew I and Ungar, Lyle H},
  journal={Machine Learning},
  volume={68},
  number={3},
  pages={235--265},
  year={2007},
  publisher={Springer}
}

@article{abbass2002evolutionary,
  title={An evolutionary artificial neural networks approach for breast cancer diagnosis},
  author={Abbass, Hussein A},
  journal={Artificial Intelligence in Medicine},
  volume={25},
  number={3},
  pages={265--281},
  year={2002},
  publisher={Elsevier}
}

%%%%%%%%%%

@inproceedings{kleinberg2008multi,
  title={Multi-armed bandits in metric spaces},
  author={Kleinberg, Robert and Slivkins, Aleksandrs and Upfal, Eli},
  booktitle={Proceedings of the 40th annual ACM symposium on Theory of computing},
  pages={681--690},
  year={2008},
  organization={ACM}
}

@article{bubeck2011x,
  title={X-armed bandits},
  author={Bubeck, S{\'e}bastien and Munos, R{\'e}mi and Stoltz, Gilles and Szepesvari, Csaba},
  journal={The Journal of Machine Learning Research},
  volume={12},
  pages={1655--1695},
  year={2011},
  publisher={JMLR. org}
}


%IMAGE MINING PAPERS

@article{borgstede2004radpeer,
  title={RADPEER quality assurance program: a multifacility study of interpretive disagreement rates},
  author={Borgstede, James P and Lewis, Rebecca S and Bhargavan, Mythreyi and Sunshine, Jonathan H},
  journal={Journal of the American College of Radiology},
  volume={1},
  number={1},
  pages={59--65},
  year={2004},
  publisher={Elsevier}
}

@article{johnson2009developing,
  title={Developing a Radiology Quality and Safety Program: A Primer1},
  author={Johnson, C Daniel and Krecke, Karl N and Miranda, Rafael and Roberts, Catherine C and Denham, Charles},
  journal={Radiographics},
  volume={29},
  number={4},
  pages={951--959},
  year={2009},
  publisher={Radiological Society of North America}
}

@inproceedings{zhang2001image,
  title={Image mining: Issues, frameworks and techniques},
  author={Zhang, Ji and Hsu, Wynne and Lee, Mong Li},
  booktitle={Proceedings of the 2nd ACM SIGKDD International Workshop on Multimedia Data Mining (MDM/KDD'01)},
  year={2001},
  organization={University of Alberta}
}

@article{vailaya2001image,
  title={Image classification for content-based indexing},
  author={Vailaya, Aditya and Figueiredo, M{\'a}rio AT and Jain, Anil K and Zhang, Hong-Jiang},
  journal={Image Processing, IEEE Transactions on},
  volume={10},
  number={1},
  pages={117--130},
  year={2001},
  publisher={IEEE}
}

@inproceedings{wang1997system,
  title={System for screening objectionable images using daubechies' wavelets and color histograms},
  author={Wang, James Ze and Wiederhold, Gio and Firschein, Oscar},
  booktitle={Interactive Distributed Multimedia Systems and Telecommunication Services},
  pages={20--30},
  year={1997},
  organization={Springer}
}

@inproceedings{fan1999application,
  title={The application of AdaBoost for distributed, scalable and on-line learning},
  author={Fan, Wei and Stolfo, Salvatore J and Zhang, Junxin},
  booktitle={Proceedings of the fifth ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={362--366},
  year={1999},
}

@inproceedings{zaiane1998mining,
  title={Mining multimedia data},
  author={Za{\"\i}ane, Osmar R and Han, Jiawei and Li, Ze-Nian and Hou, Jean},
  booktitle={Proceedings of the 1998 conference of the Centre for Advanced Studies on Collaborative research},
  pages={24},
  year={1998},
  organization={IBM Press}
}

@article{jain1999data,
  title={Data clustering: a review},
  author={Jain, Anil K and Murty, M Narasimha and Flynn, Patrick J},
  journal={ACM computing surveys (CSUR)},
  volume={31},
  number={3},
  pages={264--323},
  year={1999},
  publisher={Acm}
}

@article{bruzzone2001unsupervised,
  title={Unsupervised retraining of a maximum likelihood classifier for the analysis of multitemporal remote sensing images},
  author={Bruzzone, Lorenzo and Prieto, Diego Fern{\`a}ndez},
  journal={Geoscience and Remote Sensing, IEEE Transactions on},
  volume={39},
  number={2},
  pages={456--460},
  year={2001},
  publisher={IEEE}
}

@inproceedings{megalooikonomou1999mining,
  title={Mining lesion-deficit associations in a brain image database},
  author={Megalooikonomou, Vasileios and Davatzikos, Christos and Herskovits, Edward H},
  booktitle={Proceedings of the fifth ACM SIGKDD international conference on Knowledge discovery and data mining},
  pages={347--351},
  year={1999},
  organization={ACM}
}

@inproceedings{zaiane1998mining,
  title={Mining multimedia data},
  author={Za{\"\i}ane, Osmar R and Han, Jiawei and Li, Ze-Nian and Hou, Jean},
  booktitle={Proceedings of the 1998 conference of the Centre for Advanced Studies on Collaborative research},
  pages={24},
  year={1998},
  organization={IBM Press}
}

@book{haykin1994neural,
  title={Neural networks: a comprehensive foundation},
  author={Haykin, Simon},
  year={1994},
  publisher={Prentice Hall PTR}
}

@article{gardner1996automatic,
  title={Automatic detection of diabetic retinopathy using an artificial neural network: a screening tool.},
  author={Gardner, GG and Keating, D and Williamson, TH and Elliott, AT},
  journal={British journal of Ophthalmology},
  volume={80},
  number={11},
  pages={940--944},
  year={1996},
  publisher={BMJ Publishing Group Ltd.}
}


%BREAST CANCER PAPERS


@article{mangasarian1995breast,
  title={Breast cancer diagnosis and prognosis via linear programming},
  author={Mangasarian, Olvi L and Street, W Nick and Wolberg, William H},
  journal={Operations Research},
  volume={43},
  number={4},
  pages={570--577},
  year={1995},
  publisher={INFORMS}
}

@article{ciatto1997benign,
  title={Benign breast surgical biopsies: are they always justified?},
  author={Ciatto, S and Bonardi, R and Ravaioli, A and Canuti, D and Foglietta, F and Modena, S and Zanconati, F and Cressa, C and Ferrara, P and Marrazzo, A},
  journal={Tumori},
  volume={84},
  number={5},
  pages={521--524},
  year={1997}
}

@misc{Bache+Lichman:2013 ,
author = "K. Bache and M. Lichman",
year = "2013",
title = "{UCI} Machine Learning Repository",
url = "http://archive.ics.uci.edu/ml",
institution = "University of California, Irvine, School of Information and Computer Sciences" }

%%%%%%

%ACTIVE LEARNING REFERENCES

@article{settles2010active,
  title={Active learning literature survey},
  author={Settles, Burr},
  journal={University of Wisconsin, Madison},
  volume={52},
  pages={55--66},
  year={2010}
}

@article{freund1997selective,
  title={Selective sampling using the query by committee algorithm},
  author={Freund, Yoav and Seung, H Sebastian and Shamir, Eli and Tishby, Naftali},
  journal={Machine learning},
  volume={28},
  number={2-3},
  pages={133--168},
  year={1997},
  publisher={Springer}
}


@inproceedings{gilad2005query,
  title={Query by committee made real},
  author={Gilad-Bachrach, Ran and Navot, Amir and Tishby, Naftali},
  booktitle={NIPS},
  volume={5},
  pages={443--450},
  year={2005}
}

@incollection{dasgupta2005analysis,
  title={Analysis of perceptron-based active learning},
  author={Dasgupta, Sanjoy and Kalai, Adam Tauman and Monteleoni, Claire},
  booktitle={Learning Theory},
  pages={249--263},
  year={2005},
  publisher={Springer}
}




@article{cesa1997use,
  title={How to use expert advice},
  author={Cesa-Bianchi, Nicolo and Freund, Yoav and Haussler, David and Helmbold, David P and Schapire, Robert E and Warmuth, Manfred K},
  journal={Journal of the ACM (JACM)},
  volume={44},
  number={3},
  pages={427--485},
  year={1997},
  publisher={ACM}
}

@inProceedings{chai2002bayesian,
  title={Bayesian online classifiers for text classification and filtering},
  author={Chai, Kian Ming Adam and Chieu, Hai Leong and Ng, Hwee Tou},
  booktitle={Proc. of the 25th annual international ACM SIGIR conference on research and development in information retrieval},
  pages={97--104},
  year={2002},
  organization={ACM}
}




@inProceedings{ishibashi2005detecting,
  title={Detecting mass-mailing worm infected hosts by mining DNS traffic data},
  author={Ishibashi, Keisuke and Toyono, Tsuyoshi and Toyama, Katsuyasu and Ishino, Masahiro and Ohshima, Haruhiko and Mizukoshi, Ichiro},
  booktitle={Proc. of the 2005 ACM SIGCOMM workshop on Mining network data},
  pages={159--164},
  year={2005},
  organization={ACM}
}

@inProceedings{yubig2013,
  title={A Fast Online Learning Algorithm for Distributed Mining of BigData},
  author={Y. Zhang, D. Sow, D. Turaga and M. van der Schaar},
  booktitle={the Big Data Analytics workshop at SIGMETRICS 2013},
  year={2013},
}



@article{buhlmann2003boosting,
  title={Boosting with the L 2 loss: regression and classification},
  author={B{\"u}hlmann, Peter and Yu, Bin},
  journal={Journal of the American Statistical Association},
  volume={98},
  number={462},
  pages={324--339},
  year={2003},
  publisher={American Statistical Association}
}

@inProceedings{lazarevic2001distributed,
  title={The distributed boosting algorithm},
  author={Lazarevic, Aleksandar and Obradovic, Zoran},
  booktitle={Proc. of the seventh ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={311--316},
  year={2001},
  organization={ACM}
}

@article{perlich2011cross,
  title={On cross-validation and stacking: Building seemingly predictive models on random data},
  author={Perlich, Claudia and {\'S}wirszcz, Grzegorz},
  journal={ACM SIGKDD Explorations Newsletter},
  volume={12},
  number={2},
  pages={11--15},
  year={2011},
  publisher={ACM}
}









%DISTRIBUTED DATA MINING PAPERS 5.14.2013
@InProceedings{tekin2012sequencing,
author = "C. Tekin and M. Liu",
title = {{Online learning in decentralized multi-user spectrum access with synchronized explorations}},
booktitle= "Proc. of IEEE MILCOM 2012",
year = "2012",
}

@article{crammer2011multiclass,
  title={Multiclass classification with bandit feedback using adaptive regularization},
  author={Crammer, Koby and Gentile, Claudio},
  year={2011}
}




@article{predd2006distributed,
  title={Distributed learning in wireless sensor networks},
  author={Predd, Joel B and Kulkarni, SB and Poor, H Vincent},
  journal={Signal Processing Magazine, IEEE},
  volume={23},
  number={4},
  pages={56--69},
  year={2006},
  publisher={IEEE}
}

@article{perez2010robust,
  title={Robust and low complexity distributed kernel least squares learning in sensor networks},
  author={P{\'e}rez-Cruz, Fernando and Kulkarni, Sanjeev R},
  journal={Signal Processing Letters, IEEE},
  volume={17},
  number={4},
  pages={355--358},
  year={2010},
  publisher={IEEE}
}

@article{breiman1996bagging,
  title={Bagging predictors},
  author={Breiman, Leo},
  journal={Machine learning},
  volume={24},
  number={2},
  pages={123--140},
  year={1996},
  publisher={Springer}
}

@article{wolpert1992stacked,
  title={Stacked generalization},
  author={Wolpert, David H},
  journal={Neural networks},
  volume={5},
  number={2},
  pages={241--259},
  year={1992},
  publisher={Elsevier}
}

@article{mateos2010distributed,
  title={Distributed sparse linear regression},
  author={Mateos, Gonzalo and Bazerque, Juan Andr{\'e}s and Giannakis, Georgios B},
  journal={Signal Processing, IEEE Transactions on},
  volume={58},
  number={10},
  pages={5262--5276},
  year={2010},
  publisher={IEEE}
}

@article{chen2004channel,
  title={Channel aware decision fusion in wireless sensor networks},
  author={Chen, Biao and Jiang, Ruixiang and Kasetkasem, Teerasit and Varshney, Pramod K},
  journal={Signal Processing, IEEE Transactions on},
  volume={52},
  number={12},
  pages={3454--3458},
  year={2004},
  publisher={IEEE}
}

@article{blum1997empirical,
  title={Empirical support for winnow and weighted-majority algorithms: Results on a calendar scheduling domain},
  author={Blum, Avrim},
  journal={Machine Learning},
  volume={26},
  number={1},
  pages={5--23},
  year={1997},
  publisher={Springer}
}

@article{kargupta1999collective,
  title={Collective data mining: A new perspective toward distributed data mining},
  author={Kargupta, Hillol and Park, B and Hershberger, Daryl and Johnson, Erik},
  journal={Advances in Distributed and Parallel Knowledge Discovery},
  number={part II},
  pages={131--174},
  year={1999},
  publisher={Citeseer}
}

@article{bartlett2008high,
  title={High-probability regret bounds for bandit online linear optimization},
  author={Bartlett, Peter L and Dani, Varsha and Hayes, Thomas and Kakade, Sham and Rakhlin, Alexander and Tewari, Ambuj},
  year={2008}
}

@article{gai2012combinatorial,
  title={Combinatorial network optimization with unknown variables: Multi-armed bandits with linear rewards and individual observations},
  author={Gai, Yi and Krishnamachari, Bhaskar and Jain, Rahul},
  journal={IEEE/ACM Transactions on Networking (TON)},
  volume={20},
  number={5},
  pages={1466--1478},
  year={2012},
  publisher={IEEE Press}
}

@article{sewell2008ensemble,
  title={Ensemble learning},
  author={Sewell, Martin},
  journal={RN},
  volume={11},
  number={02},
  year={2008}
}

@article{zheng2011attribute,
  title={Attribute-distributed learning: models, limits, and algorithms},
  author={Zheng, Haipeng and Kulkarni, Sanjeev R and Poor, HVincent},
  journal={Signal Processing, IEEE Transactions on},
  volume={59},
  number={1},
  pages={386--398},
  year={2011},
  publisher={IEEE}
}



@book{alpaydin2004introduction,
  title={Introduction to machine learning},
  author={Alpaydin, Ethem},
  year={2004},
  publisher={The MIT Press}
}

@inProceedings{mcconnell2004building,
  title={Building predictors from vertically distributed data},
  author={McConnell, Sabine and Skillicorn, David B},
  booktitle={Proc. of the 2004 conference of the Centre for Advanced Studies on Collaborative research},
  pages={150--162},
  year={2004},
  organization={IBM Press}
}


















%6/22/11 - NEW REFERENCES FOR ALLERTON 2011 PAPER

@ARTICLE{lewis2002,
author = "M. E. Lewis and M. L. Puterman",
title = "Bias Optimality",
journal = "International Series in Operations Research and Management Science",
issue = "40",
pages = "89-112",
year = "2002",
}

@ARTICLE{burnetas1997,
author = "A. N. Burnetas and M. N. Katehakis",
title = "Optimal Adaptive Policies for Markov Decision Processes",
journal = "Mathematics of Operations Research",
volume = "22",
number = "1",
pages = "222-255",
year = "1997",
}

@ARTICLE{tewari2008,
author = "A. Tewari and P. Bartlett",
title = "Optimistic Linear Programming Gives Logarithmic Regret for Irreducible MDPs",
journal = "Advances in Neural Information Processing Systems",
volume = "20",
pages = "1505-1512",
year = "2008",
}

@ARTICLE{platzman1980,
author = "L. K. Platzman",
title = "Optimal Infinite-Horizon Undiscounted Control of Finite Probabilistic Systems",
journal = "SIAM J. Control Optim.",
volume = "18",
pages = "362-380",
year = "1980",
}

@ARTICLE{hsu2006,
author = "S. P. Hsu and D. M. Chuang and A. Arapostathis",
title = "On the existence of stationary optimal policies for partially observed MDPs under the long-run average cost criterion",
journal = "Systems and Control Letters",
volume = "55",
pages = "165-173",
year = "2006",
}

@ARTICLE{mitrophanov2005,
author = "A. Y. Mitrophanov",
title = "Senstivity and Convergence of Uniformly Ergodic Markov Chains",
journal = "J. Appl. Prob.",
volume = "42",
pages = "1003-1014",
year = "2005",
}

@ARTICLE{papadim1999,
author = "C. H. Papadimitriou and J. N. Tsitsiklis",
title = "The complexity of optimal queuing network control",
journal = "Math. Oper. Res.",
volume = "24",
number ="2",
pages = "293-305",
year = "1999",
}





%Infocom-submission
@ARTICLE{zhao,
author = "Q. Zhao and B. Sadler",
title = "A survey of dynamic spectrum access",
journal = "IEEE Signal Processing Magazine: Special Issue on Resource-Constrained Signal Processing, Communications, and Networking",
volume = "24",
pages = "79-89",
month = "May",
year = "2007",
}

@ARTICLE{hliu1,
author = "H. Liu and K. Liu and Q. Zhao",
title = "Learning in a Changing World: Non-Bayesian Restless Multi-Armed Bandit",
journal = "Techinal Report, UC Davis",
month = "October",
year = "2010",
}

@ARTICLE{hliu2,
author = "H. Liu and K. Liu and Q. Zhao",
title = "Distributed Learning in Multi-armed Bandit with Multiple Players - Markovian Rewards",
journal = "Techinal Report, UC Davis",
month = "October",
year = "2010",
}


@ARTICLE{robbins2,
author = "H. Robbins",
title = "Some aspects of the sequential design of experiments",
journal = "Bull. Amer. Math. Soc.",
volume = "55",
pages = "527-535",
year = "1952",
}

@ARTICLE{auer2,
author = "P. Auer and N. Cesa-Bianchi and Y. Freund and R.E. Schapire",
title = "The nonstochastic multiarmed bandit problem",
journal = "SIAM Journal on Computing",
volume = "32",
pages = "48-77",
year = "2002",
}

@ARTICLE{lai1,
author = "T. Lai and H. Robbins",
title = "Asymptotically efficient adaptive allocation rules",
journal = "Advances in Applied Mathematics",
volume = "6",
pages = "4-22",
year = "1985",
}

@ARTICLE{anantharam2,
author = "V. Anantharam and P. Varaiya and J . Walrand",
title = "Asymptotically efficient allocation rules for the multiarmed bandit problem with multiple plays-Part I: IID rewards",
journal = "IEEE Trans. Automat. Contr.",
pages = "968-975",
month = "November",
year = "1987",
}

@ARTICLE{anantharam1,
author = "V. Anantharam and P. Varaiya and J . Walrand",
title = "Asymptotically efficient allocation rules for the multiarmed bandit problem with multiple plays-Part II: Markovian rewards",
journal = "IEEE Trans. Automat. Contr.",
pages = "977-982",
month = "November",
year = "1987",
}

@ARTICLE{agrawal1,
author = "R. Agrawal",
title = "Sample Mean Based Index Policies with O(log n) Regret for the Multi-Armed Bandit Problem",
journal = "Advances in Applied Probability",
volume = "27",
number = "4",
pages = "1054-1078",
month = "December",
year = "1995",
}

@ARTICLE{auer,
author = "P. Auer and N. Cesa-Bianchi and P. Fischer",
title = "Finite-time analysis of the multiarmed bandit problem",
journal = "Machine Learning",
volume = "47",
pages = "235–256",
year = "2002",
}

@article{chlebus2009approximate,
  title={An approximate formula for a partial sum of the divergent p-series},
  author={Chlebus, Edward},
  journal={Applied Mathematics Letters},
  volume={22},
  number={5},
  pages={732--737},
  year={2009},
  publisher={Elsevier}
}



@ARTICLE{liu2,
author = "K. Liu and Q. Zhao",
title = "Distributed Learning in Multi-Armed Bandit with Multiple Players, http://arxiv.org/abs/0910.2065",
}

@InProceedings{anandkumar,
author = "A. Anandkumar and N. Michael and A.K. Tang",
title = "Opportunistic spectrum access with multiple players: Learning under competition",
booktitle = "Proc. of IEEE INFOCOM",
month = "March",
year = "2010",
}

@article{slivkins2009contextual,
  title={Contextual bandits with similarity information},
  author={Slivkins, Aleksandrs},
  journal={arXiv preprint arXiv:0907.3986},
  year={2009}
}

@article{ortner2010exploiting,
  title={Exploiting similarity information in reinforcement learning},
  author={Ortner, Ronald},
  journal={Proceedings 2nd ICAART},
  pages={203--210},
  year={2010}
}
@article{liu2010distributed,
  title={Distributed learning in multi-armed bandit with multiple players},
  author={Liu, Keqin and Zhao, Qing},
  journal={Signal Processing, IEEE Transactions on},
  volume={58},
  number={11},
  pages={5667--5681},
  year={2010},
  publisher={IEEE}
}





@article{dudik2011efficient,
  title={Efficient optimal learning for contextual bandits},
  author={Dudik, Miroslav and Hsu, Daniel and Kale, Satyen and Karampatziakis, Nikos and Langford, John and Reyzin, Lev and Zhang, Tong},
  journal={arXiv preprint arXiv:1106.2369},
  year={2011}
}

@article{langford2007epoch,
  title={The epoch-greedy algorithm for contextual multi-armed bandits},
  author={Langford, John and Zhang, Tong},
  journal={Advances in Neural Information Processing Systems},
  volume={20},
  pages={1096--1103},
  year={2007},
  publisher={Citeseer}
}

@inProceedings{chu2011contextual,
  title={Contextual bandits with linear payoff functions},
  author={Chu, Wei and Li, Lihong and Reyzin, Lev and Schapire, Robert E},
  booktitle={Proc. of the International Conference on Artificial Intelligence and Statistics (AISTATS)},
  year={2011}
}

@inProceedings{li2010contextual,
  title={A contextual-bandit approach to personalized news article recommendation},
  author={Li, Lihong and Chu, Wei and Langford, John and Schapire, Robert E},
  booktitle={Proc. of the 19th international conference on World wide web},
  pages={661--670},
  year={2010},
  organization={ACM}
}












@ARTICLE{gittins1,
author = "J.C. Gittins",
title = "Bandit Processes and Dynamic Allocation Indices",
journal = "Journal of the Royal Statistical Society",
series = "B",
volume = "41",
number = "2",
pages = "148-177",
year = "1979",
}

@ARTICLE{gillman,
author = "D. Gillman",
title = "A chernoff bound for random walks on expander graphs",
journal = "SIAM J. Comp.",
volume = "27",
number = "4",
pages = "1203–1220",
year = "1998",
}

@ARTICLE{lezaud,
author = "Q. Zhao and B. Sadler",
title = "Chernoff-type Bound for Finite Markov Chains",
journal = "Ann. Appl. Prob.",
volume = "8",
pages = "849-867",
year = "1998",
}

@ARTICLE{ahmad,
author = "S. H. A. Ahmad and M. Liu and T. Javidi and Q. Zhao and B. Krishnamachari",
title = "Optimality of Myopic Sensing in Multi-Channel Opportunistic Access",
journal = "IEEE Transactions on Information Theory",
volume = "55",
number = "9",
pages = "4040-4050",
month = "September",
year = "2009",
}

@ARTICLE{guha,
author = "S. Guha and K. Mungala and P. Shi",
title = "Approximation Algorithms for Restless Bandit Problems",
journal = "20th ACM-SIAM Symp. on Discrete Algorithms (SODA)",
pages = "28-37",
year = "2009",
}

@InProceedings{tekin1,
author = "C. Tekin and M. Liu",
title = "Online Algorithms for the Multi-Armed Bandit Problem with Markovian Rewards",
booktitle = "Proc. of the 48th Annual Allerton Conference on Communication, Control, and Computation",
month="September",
year="2010",
}

@InProceedings{tekin2,
author = "C. Tekin and M. Liu",
title = "Online Learning in Opportunistic Spectrum Access: A Restless Bandit Approach",
booktitle = "30th IEEE International Conference on Computer Communications (INFOCOM)",
month="April",
year="2011",
}

@ARTICLE{tekin3,
author = "C. Tekin and M. Liu",
title = "Online Learning of Rested and Restless Bandits",
journal = "http://arxiv.org/abs/1102.3508v1",
}

@InProceedings{tekin4,
author = "C. Tekin and M. Liu",
title = "Performance and Convergence of Multi-user Online Learning",
booktitle = "2nd International ICST Conference on Game Theory for Networks (GAMENETS)",
month="April",
year="2011",
}


@ARTICLE{whittle,
author = "P. Whitlle",
title = "Restless Bandits",
journal = "J. Appl. Prob.",
pages = "301-313",
year = "1988",
}

@InProceedings{krishnamachari, 
author = "Y. Gai and B. Krishnamachari and R. Jain", 
title = "Learning multiuser channel allocations in cognitive radio networks: a combinatorial multi-armed bandit formulation", 
booktitle = "IEEE Symp. on Dynamic Spectrum Access Networks (DySPAN)", 
month = "April",
year = "2010",
} 

@InProceedings{geirhofer,
author = "S. Geirhofer and L. Tong and B. Sadler",
title = "A measurement-based model for dynamic spectrum access in WLAN channels",
booktitle = "IEEE Military Communication Conf.",
year = "2006",
}

@BOOK{bremaud,
author = "P. Bremaud",
title = "Markov Chains, Gibbs Fields, Monte Carlo Simulation and Queues",
year = "1998",
publisher = "Springer",
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%DATA MINING REFERENCES

%Concept Drift

@article{minku2010impact,
  title={The impact of diversity on online ensemble learning in the presence of concept drift},
  author={Minku, Leandro L and White, Allan P and Yao, Xin},
  journal={Knowledge and Data Engineering, IEEE Transactions on},
  volume={22},
  number={5},
  pages={730--742},
  year={2010},
  publisher={IEEE}
}

@article{minku2012ddd,
  title={DDD: A new ensemble approach for dealing with concept drift},
  author={Minku, Leandro L and Yao, Xin},
  journal={Knowledge and Data Engineering, IEEE Transactions on},
  volume={24},
  number={4},
  pages={619--633},
  year={2012},
  publisher={IEEE}
}

@inProceedings{narasimhamurthy2007framework,
  title={A framework for generating data to simulate changing environments},
  author={Narasimhamurthy, Anand and Kuncheva, Ludmila I},
  booktitle={Proceedings of the 25th conference on Proceedings of the 25th IASTED International Multi-Conference: artificial intelligence and applications},
  volume={549},
  pages={389},
  year={2007},
  organization={ACTA Press}
}

@incollection{gama2004learning,
  title={Learning with drift detection},
  author={Gama, Joao and Medas, Pedro and Castillo, Gladys and Rodrigues, Pedro},
  booktitle={Advances in Artificial Intelligence--SBIA 2004},
  pages={286--295},
  year={2004},
  publisher={Springer}
}

@inProceedings{gao2007appropriate,
  title={On appropriate assumptions to mine data streams: Analysis and practice},
  author={Gao, Jing and Fan, Wei and Han, Jiawei},
  booktitle={Data Mining, 2007. ICDM 2007. Seventh IEEE International Conference on},
  pages={143--152},
  year={2007},
  organization={IEEE}
}

@article{baena2006early,
  title={Early drift detection method},
  author={Baena-Garc{\'\i}a, Manuel and del Campo-{\'A}vila, Jos{\'e} and Fidalgo, Ra{\'u}l and Bifet, Albert and Gavald{\`a}, Ricard and Morales-Bueno, Rafael},
  year={2006}
}

@article{stanley2003learning,
  title={Learning concept drift with a committee of decision trees},
  author={Stanley, Kenneth O},
  journal={Informe t{\'e}cnico: UT-AI-TR-03-302, Department of Computer Sciences, University of Texas at Austin, USA},
  year={2003},
  publisher={Citeseer}
}

@article{kolter2007dynamic,
  title={Dynamic weighted majority: An ensemble method for drifting concepts},
  author={Kolter, J Zico and Maloof, Marcus A},
  journal={The Journal of Machine Learning Research},
  volume={8},
  pages={2755--2790},
  year={2007},
  publisher={JMLR. org}
}


@inProceedings{lienhart2003detector,
  title={A detector tree of boosted classifiers for real-time object detection and tracking},
  author={Lienhart, Rainer and Liang, Luhong and Kuranov, Alexander},
  booktitle={Proc. of International Conference on Multimedia and Expo (ICME'03) },
  volume={2},
  pages={II--277},
  year={2003},
  organization={IEEE}
}

@article{mao2005multiclass,
  title={Multiclass cancer classification by using fuzzy support vector machine and binary decision tree with gene selection},
  author={Mao, Yong and Zhou, Xiaobo and Pi, Daoying and Sun, Youxian and Wong, Stephen TC},
  journal={Journal of Biomedicine and Biotechnology},
  volume={2005},
  number={2},
  pages={160--171},
  year={2005},
  publisher={Hindawi Publishing Corporation}
}

@inProceedings{freund1995desicion,
  title={A decision-theoretic generalization of on-line learning and an application to boosting},
  author={Freund, Yoav and Schapire, Robert E},
  booktitle={Computational learning theory},
  pages={23--37},
  year={1995},
  organization={Springer}
}

@book{oza2001online,
  title={Online ensemble learning},
  author={Oza, Nikunj Chandrakant and Russell, Stuart},
  year={2001},
  publisher={University of California, Berkeley}
}

@inproceedings{langford2007epoch,
  title={The epoch-greedy algorithm for multi-armed bandits with side information},
  author={Langford, John and Zhang, Tong},
  booktitle={Advances in neural information processing systems},
  pages={817--824},
  year={2007}
}

@inproceedings{lu2010contextual,
  title={Contextual multi-armed bandits},
  author={Lu, Tyler and P{\'a}l, D{\'a}vid and P{\'a}l, Martin},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={485--492},
  year={2010}
}

@inproceedings{crammer2010regret,
  title={Regret Minimization With Concept Drift.},
  author={Crammer, Koby and Mansour, Yishay and Even-Dar, Eyal and Vaughan, Jennifer Wortman},
  booktitle={COLT},
  pages={168--180},
  year={2010}
}



@article{tekin2012online,
  title={Online learning of rested and restless bandits},
  author={Tekin, Cem and Liu, Mingyan},
  journal={Information Theory, IEEE Transactions on},
  volume={58},
  number={8},
  pages={5588--5611},
  year={2012},
  publisher={IEEE}
}
@ARTICLE{6362216, 
 author={Haoyang Liu and Keqin Liu and Qing Zhao}, 
 journal={Information Theory, IEEE Transactions on}, 
 title={Learning in a Changing World: Restless Multiarmed Bandit With Unknown Dynamics}, 
 year={2013}, 
 volume={59}, 
 number={3}, 
 pages={1902-1916}, 
 }
 
@ARTICLE{cem2013contextdata, 
 author={Cem Tekin and Mihaela van der Schaar}, 
 journal={submitted to Signal Processing, IEEE Transactions on}, 
 title={Decentralized Online Big Data Classification - a Bandit Framework}, 
 year={2013},  
 }
 
 @ARTICLE{cem2013deccontext, 
 author={Cem Tekin and Mihaela van der Schaar}, 
 journal={submitted to Signal Processing, IEEE Transactions on}, 
 title={Online Learning in Decentralized Contextual Bandits}, 
 year={2013},  
 }
 
 @article{shalev2011pegasos,
  title={Pegasos: Primal estimated sub-gradient solver for svm},
  author={Shalev-Shwartz, Shai and Singer, Yoram and Srebro, Nathan and Cotter, Andrew},
  journal={Mathematical Programming},
  volume={127},
  number={1},
  pages={3--30},
  year={2011},
  publisher={Springer}
}

@inproceedings{littlestone1989weighted,
  title={The weighted majority algorithm},
  author={Littlestone, Nick and Warmuth, Manfred K},
  booktitle={Foundations of Computer Science, 1989., 30th Annual Symposium on},
  pages={256--261},
  year={1989},
  organization={IEEE}
}

@article{littlestone1988learning,
  title={Learning quickly when irrelevant attributes abound: A new linear-threshold algorithm},
  author={Littlestone, Nick},
  journal={Machine learning},
  volume={2},
  number={4},
  pages={285--318},
  year={1988},
  publisher={Springer}
}

@inProceedings{yu2013fast,
  title={A Fast Online Learning Algorithm for Distributed Mining of BigData},
  author={Zhang, Yu and Sow, Daby and Turaga, Deepak and van der Schaar, Mihaela},
  booktitle={Proc. of the Big Data Analytics workshop at SIGMETRICS},
  year={2013},
}

@article{tekin2013arxivbig,
  title={Decentralized Online Big Data Classification - a Bandit Framework},
  author={Tekin, Cem and van der Schaar, Mihaela},
  journal={arXiv preprint arXiv:1308.4565},
  year={2013}
}

%PAPERS MENTIONED BY THE REVIEWERS

@inproceedings{kar2011bandit,
  title={Bandit problems in networks: Asymptotically efficient distributed allocation rules},
  author={Kar, Soummya and Poor, H Vincent and Cui, Shuguang},
  booktitle={Decision and Control and European Control Conference (CDC-ECC), 2011 50th IEEE Conference on},
  pages={1771--1778},
  year={2011},
  organization={IEEE}
}

@inproceedings{szorenyi2013gossip,
  title={Gossip-based distributed stochastic bandit algorithms},
  author={Sz{\"o}r{\'e}nyi, Bal{\'a}zs and Busa-Fekete, R{\'o}bert and Hegedus, Istv{\'a}n and Orm{\'a}ndi, R{\'o}bert and Jelasity, M{\'a}rk and K{\'e}gl, Bal{\'a}zs},
  booktitle={Proceedings of the 30th International Conference on Machine Learning},
  year={2013}
}

@incollection{hazan2007online,
  title={Online learning with prior knowledge},
  author={Hazan, Elad and Megiddo, Nimrod},
  booktitle={Learning theory},
  pages={499--513},
  year={2007},
  publisher={Springer}
}

@incollection{masud2009integrating,
  title={Integrating novel class detection with classification for concept-drifting data streams},
  author={Masud, Mohammad M and Gao, Jing and Khan, Latifur and Han, Jiawei and Thuraisingham, Bhavani},
  booktitle={Machine Learning and Knowledge Discovery in Databases},
  pages={79--94},
  year={2009},
  publisher={Springer}
}






















==> algoanalysis2.tex <==
\begin{lemma} \label{lemma:exploitbound}
Let $\xi_{i,t} =  L l(p_{i,t})$. With probability at least $1-\delta$ the total regret in exploitation slots is bounded above by 
\begin{align}
2(C_2 +1) L \sum_{t \in \tau(T)} ( l(p_{c(\alpha_t),t} + l(p_{c(a^*(\boldsymbol{x}_t)),t}   )   ) ,    \notag
\end{align}
and the instantaneous regret at every time step $t \in \tau(T)$ is bounded above by
\begin{align}
2(C_2 +1) L  ( l(p_{c(\alpha_t),t} + l(p_{c(a^*(\boldsymbol{x}_t)),t}   )   ).     \notag
\end{align}
The total regret in exploration slots is bounded by 
\begin{align}
\left( A L_2 \log(t A D/ \delta) /L^2 + A \right) 
 \sum_{i \in {\cal D}} \sum_{l=1}^\infty J_{i,l}(T) 2^{2l} ,    \notag
\end{align}
where $J_{i,l}(T)$ is the number of type $i$ and level $l$ intervals activated by time $T$. 
\end{lemma}
\begin{proof}
Since for $t \in \tau(T)$, $\alpha_t = \argmax_{a \in {\cal A}} \bar{r}^{\hat{c}_t(a)}_t (p_{\hat{c}_t(a),t}, a) $,
using the result of Lemma \ref{lemma:estimatedrel}, we conclude that
\begin{align}
 \mu_t(\alpha_t) &\geq \mu_t(a^*(\boldsymbol{x}_t)) - (2 C_2 + 1) ( l(p_{c(\alpha_t),t} + l(p_{c(a^*(\boldsymbol{x}_t)),t}   )  - \xi_{c(\alpha_t),t} - \xi_{c(a^*(\boldsymbol{x}_t)),t}      \notag \\
 & = (2 C_2 + 2) ( l(p_{c(\alpha_t),t} + l(p_{c(a^*(\boldsymbol{x}_t)),t}   )  ,
\end{align}
The bound for explorations follows from the fact that 
\begin{align}
S^{\textrm{ind}(q)}_t(q,a) \leq\frac{L_2 \log(t A D / \delta)}{\xi^2_{i,t}} +1,      \notag
\end{align}
at all times $t$, for all $a \in {\cal A}$ and $q \in Q_i(t) $.

\end{proof}

==> dummydescripton.tex <==
At each exploitation step, CALIF computes the sample mean reward of action $a$ for each interval $i \in {\cal D}$ as 
\begin{align}
\bar{r}^{i}_t(p_{i,t},a)  = \frac{ \sum_{p_{j}\in{\cal P}_{j}(t)}  \bar{r}^{ij}_t(p_i,p_j,a)  S^{ij}_t(p_i,p_j,a) }
{ \sum_{p_{j}\in{\cal P}_{j}(t)} S^{ij}_t(p_i,p_j,a)  } . 
\end{align}

Let $\boldsymbol{p}_{-ij}$ be the vector of intervals in $\boldsymbol{p}$ with intervals for $i$th and $j$th types of contexts excluded, let $\boldsymbol{p}_{ij} = (p_i, p_j)$ be a pair of intervals for $i$th and $j$th types of contexts.
The interval corresponding to type $k \in \{i,j\}$ context in $\boldsymbol{p}_{ij}$ is denoted by $\boldsymbol{p}_{ij}(k)$.
Let 
$(\boldsymbol{p}'_{-ij}, \boldsymbol{p}_{ij})$ denote the vector of intervals where the pair of $i$th and $j$th elements is $\boldsymbol{p}_{ij}$ and other elements come from $\boldsymbol{p}'_{-ij}$.
The set of all interval pairs in ${\cal P}(t)$ is denoted by ${\cal Q}(t)$.

For $a\in{\cal A}$, let $\bar{r}_{t}(\boldsymbol{p},a)$ be the
{\em joint sample mean reward} of taking action $a$ at times when the
context vector is in set $\boldsymbol{p}$ by time $t$. 
Similarly, let $\bar{r}_{t}^{ij}(\boldsymbol{p}_{ij}, a)$
be the {\em pairwise sample mean reward} of taking action $a$ at times
when the type $i$ and type $j$ context pair is in interval pair $\boldsymbol{p}_{ij}$ by time $t$.
Let $\bar{r}_{t}^{i}(p_{i},a$) be
the {\em marginal sample mean reward} of taking action $a$ at times when
type $i$ context is in set $p_{i}$ by time $t$. 
We have

\begin{align*}
\bar{r}_{t}^{i}(p_{i},a) 
&= \frac{ \sum_{p_{j}\in{\cal P}_{j}(t)} \sum_{ \boldsymbol{p}'_{-ij} } \bar{r}_{t}( ( \boldsymbol{p}'_{-ij}, p_i, p_j ) , a ) S_{t}( ( \boldsymbol{p}'_{-ij}, p_i, p_j ) ,a ) }
{ \sum_{ p_{j} \in {\cal P}_{j}(t) } \sum_{ \boldsymbol{p}'_{-ij} } S_{t}((\boldsymbol{p}'_{-ij}, p_i, p_j),a) } ,
\end{align*}
and
\begin{align*}
\bar{r}^{ij}_t(p_i,p_j,a) 
&= \frac{\sum_{ \boldsymbol{p}_{-ij} } \bar{r}_{t}( ( \boldsymbol{p}'_{-ij}, p_i, p_j ), a ) S_{t}(\boldsymbol{p}_{-ij},a)}
{\sum_{\boldsymbol{p}_{-ij}} S_{t}( \boldsymbol{p}'_{-ij}, p_i, p_j ),a)} .
\end{align*}
Since we have
\begin{align}
S^{ij}_t(p_i,p_j,a) &= \sum_{\boldsymbol{p}_{-ij}} S_{t}(( \boldsymbol{p}'_{-ij}, p_i, p_j ),a)  ,    \notag
\end{align}
we can write
Since we know that for each action there is a single type of relevant context, CALIF only needs to store marginal and pairwise counters and sample mean rewards in order to operate. 
Hence, its computational complexity does not depend on $D$. 

For an action $a$, in order to determine if a type $i$ context is relevant or not, CALIF compares pairwise sample means.  
Since it is known that the reward of an action only depends on one type of context, given two pairwise sample means $\bar{r}^{ij}_t(p_i,p,a)$ and $\bar{r}^{ij}_t(p_i,p',a)$ for $p \neq p' \in {\cal P}_j(t)$, if $i = c(a)$, when $S^{ij}_t(p_i,p,a)$ and $S^{ij}_t(p_i,p',a)$ are large enough, we must have
\begin{align}
 |\bar{r}^{ij}_t(p_i,p,a) - \bar{r}^{ij}_t(p_i,p',a)|  \leq L (l(p_i) + l(p_j)) ,   \label{eqn:pairwise}
\end{align}
with a high probability. 



Thus, the idea is to compare pairwise differences for context pairs that are observed enough number of times, and try to identify the type of context that is relevant to each action. 
Due to undersampling, or worst case context arrivals, it may not be always possible to identify one type of relevant context. 
There can be context that cannot be ruled about by pairwise comparisons. 
If there are actions for which there is an opportunity to explore an undersampled context pair by taking that action, then priority is given to exploring these actions. 
Otherwise, even if an action have more than one relevant context candidates, one of them is randomly chosen and then the sample mean of all actions for their relevant candidate is calculated, and the action with the highest sample mean is chosen. 

The operation of our algorithm can be summarized as follows. 
If at any time $t$ it is possible to explore some context pair by selecting action $a$, do it.
If given the current context pairs, it is not possible to do such exploration, then calculate the relevant candidates for each action $a$.
If for an action, there are multiple relevant candidates, choose one of them randomly (equivalently we can choose the one with the highest estimated reward or the lowest estimated rewards, etc. This will not make a difference in our analysis.)
Based on its {\em guessed} relevant context, calculate the sample mean of each action, and exploit the action that gives the highest sample mean. 



We have the following set of definitions
\begin{itemize}
\item $c(a)$: context relevant to action $a$.
\item $\mu(a,x_{c(a)})$: expected reward of action $a$.
\item $a^*(\boldsymbol{x}) = \argmax_{a \in {\cal A}} \mu(a, x_{c(a)})$: optimal action.
\item $\Delta(a, \boldsymbol{x}) = \mu(a^*(\boldsymbol{x}), x_{c(a^*(\boldsymbol{x}))}) - \mu(a, x_{c(a)})$.
\item $\boldsymbol{x}_t = (x_{1,t}, \ldots, x_{D,t})$.
\item $\boldsymbol{p}_t = (p_{1,t}, \ldots, p_{D,t})$.
\item $\hat{c}_t(a)$: estimated relevant context for $a$ at time $t$.
\item $a^*_t = \argmax_{a \in {\cal A} }  \hat{\mu}_t(a, p_{\hat{c}_t(a),t}) $.
\item $\hat{\mu}^*_t = \max_{a \in {\cal A} }  \hat{\mu}_t(a, p_{\hat{c}_t(a),t})$.
\item $\hat{\Delta}_t(a) = \hat{\mu}^*_t - \hat{\mu}_t(a, p_{\hat{c}_t(a),t})$: 
\item $\bar{{\cal P}}_i(t)$: the hypercubes in ${\cal P}_i(t)$ for which there exists enough observation for at least one pairwise comparison. 
\end{itemize}


\subsection{Algorithm CALIF}

\begin{enumerate}[(1)]
\item Find $\boldsymbol{p}(t)$.
\item Calculate $Q_{i,t} := \{ (p_{i,t}, p_{j,t}) : j \in {\cal D} - \{ i \}   \}$.
\item Calculate $Q_t := \bigcup_{i \in {\cal D}} Q_{i,t}$.
\item Set $\xi_{i,t} := C_1 L l(p_{i,t})$, where $C_1>0$ is a constant that will be specified later.
\item Set $D_{i,t} := L_2  \log (t D A/\delta)/\xi^2_{i,t}$, where $L_2>0$ is a constant that will be specified later. 
\item Set ${\cal U}_{i,t} := \{ a \in {\cal A} : S^{\textrm{ind}(q)}_{t}(q,a) < D_{i,t} \textrm{ for some } q \in Q_i(t)  \}$, where $\textrm{ind}(q)$ is the index of the context types in the pair of intervals $q$. 
\item Set ${\cal U}_t := \bigcup_{i \in {\cal D}} {\cal U}_{i,t}$.
\item \textbf{If} ${\cal U}_t  \neq \emptyset$, \textbf{then} randomly select and explore an action $\alpha_t \in {\cal U}_t $.  \\
Receive and \textbf{observe} reward $r_t(\alpha_t)$.
Update the pairwise and marginal sample mean estimates and counters, i.e.,

\
for all $q \in Q_t$, 
\begin{align}
\bar{r}^{i}_{t+1}(p_{i,t},\alpha_t) =  \frac{ S^{i}_t(p_{i,t},\alpha_t) \bar{r}^{i}_{t+1}(p_{i,t},\alpha_t) +  r_t(\alpha_t) }{S^{i}_t(p_{i,t},\alpha_t) + 1}       \notag
\end{align}
\begin{align}
 S^{i}_{t+1}(p_{i,t},\alpha_t)  = S^{i}_t(p_{i,t},\alpha_t) +1 , \notag
\end{align}
for all $i \in {\cal D}$,
and
\begin{align}
\bar{r}^{\textrm{ind}(q)}_{t+1}(q,a)  &= \bar{r}^{\textrm{ind}(q)}_{t}(q,a)  ,   \notag  \\
\bar{r}^{i}_{t+1}(p_{i,t},a)  &= \bar{r}^{i}_{t}(p_{i,t},a) ,
\end{align}
and
\begin{align}
 S^{\textrm{ind}(q)}_{t+1}(q,a)  &= S^{\textrm{ind}(q)}_t(q,a) ,   \notag \\
  S^{i}_{t+1}(p_{i,t},a)  &= S^{i}_t(p_{i,t},a) ,  \notag
\end{align}
for all $q \in \boldsymbol{{\cal Q}}_t$, $i \in {\cal D}$ and $a \in {\cal A} - \{ \alpha_t \}$.
\item \textbf{Else If} ${\cal U}_t  = \emptyset$, \textbf{then} for each action, find the set of candidate relevant contexts, and choose the estimated relevant context to be the one with the minimum variation over different pairs of contexts. \\
Set 
\begin{align}
\textrm{Rel}_t(a) :=  \{  i \in {\cal D} :
 | \bar{r}^{ij}_t(p_{i,t}, p_{j,t},a) - \bar{r}^{ik}_t(p_{i,t}, p_{k,t},a)    | \leq C_2 L l(p_{i,t}), \forall j,k \in {\cal D}_{-i} \}  ,    \notag
\end{align}
be the set of candidate relevant contexts for action $a$. \\
For $i \in \textrm{Rel}_t(a) $, let 
\begin{align}
\textrm{Var}_t(i,a) := \max_{j,k \in {\cal D}_{-i}}   | \bar{r}^{ij}_t(p_{i,t}, p_{j,t},a) - \bar{r}^{ik}_t(p_{i,t}, p_{k,t},a)    | .       \notag
\end{align}
The estimated relevant context for action $a$ is 
\begin{align}
\hat{c}_t(a) = \argmin_{i \in \textrm{Rel}_t(a) } \textrm{Var}_t(i,a) .      \notag
\end{align}
\textbf{Exploit}
\begin{align}
\alpha_t = \argmax_{a \in {\cal A}} \bar{r}^{\hat{c}_t(a)}_t (p_{\hat{c}_t(a),t}, a) .       \notag
\end{align}
In an exploitation step, observation of the reward $r_t(\alpha_t)$ is not necessary.
\item Update the number of arrivals to each type of interval:
\begin{align}
N^i_{t+1}(p_{i,t}) =   N^i_{t}(p_{i,t}) + 1,     \notag
\end{align}
for all $i \in {\cal D}$. 
\item Check if there is a need to update the partition.\\
\textbf{For} $i \in {\cal D}$:\\
\textbf{If} $N^i_{t+1}(p_{i,t})  \geq B 2^{\rho l (p_{i,t})}$, create two equal sized level $ l (p_{i,t}) + 1 $ intervals $p$ and $p'$ such that $p \cup p' = p_{i,t}$, and replace them with $p_{i,t}$. Update ${\cal P}_{i,t+1} = {\cal P}_{i,t} \cup \{p.p'\} - \{ p_{i,t} \}$. Initialize the counters and sample mean of the newly created intervals to 0. \\
\textbf{Else} ${\cal P}_{i,t+1} = {\cal P}_{i,t} $.\\
\textbf{End for}
\end{enumerate}

==> experiments.tex <==
\vspace{-0.15in}
\section{Experiments} \label{sec:numerical}
\vspace{-0.1in}


We use the network intrusion data set from UCI archive \cite{hettich1999uci}. Three of the features are taken as contexts and are normalized to $[0,1]$. Hence there are three types ${\cal D} = \{ 1, 2, 3 \}$. There are $8$ classifiers that are trained with different instances from the data set. The action set of the learner is equal to the set of classifiers. 
At each time step the learner observes a $3$-dimensional context vector and selects a classifier as an action, which outputs a prediction. Our performance measure is the percentage of the number of correct predictions made till the final time.


We compare the performance of ORL-CF with state-of-the-art online ensemble learning techniques given in Table \ref{tab:ourbest}. 
Different from ORL-CF, these algorithms have access to the true labels (reward observations) at all times, and instead of choosing a single classifier to make a prediction, they combine the predictions of all classifiers to produce their final prediction.
We also simulate a benchmark algorithm that we call {\em Contextual Learning with a Single Type} (CON-S). Different from ORL-CF, CON-S forms its adaptive partition and sample mean reward estimates only on ${\cal X}_d$ for any arbitrarily chosen $d \in {\cal D}$, neglecting contexts of other types. Therefore, it is a contextual bandit algorithm for a single dimensional context space with finite number of arms. The adaptive partition of CON-S is formed using the same technique as ORL-CF, however, the partition can also be created by the methods in \cite{lu2010contextual} and \cite{slivkins2011contextual} by using the {\em doubling trick}, since those algorithms require the knowledge of the time horizon. 

Results in Table \ref{tab:ourbest} show that ORL-CF has a very small error percentage and even outperforms the ensemble learning techniques. This is due to the fact that for this data set there exists at least one classifier whose prediction is very accurate for each particular value of the context vector. Learning this {\em contextual specialization} by ORL-CF outperforms ensemble prediction. ORL-CF also outperforms CON-S, since CON-S fails to capture the dependencies of action rewards on the neglected types.
 




\begin{table*}[t!]
\centering
{\fontsize{9}{8}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Abbrev. & Name & Ref. & Parameters & Error$\%$   \\
\hline
\textbf{BC} & Single best classifier & - & - & 3.12   \\
\hline
\textbf{Ada} & Adaboost & \cite{freund1995desicion} & - & 4.82   \\
\hline
\textbf{OnAda} & Fan's Online Adaboost & \cite{fan1999application} & Window size $w=100$ & 2.69   \\
\hline
\textbf{AM} & Average Majority & \cite{gao2007appropriate} & - & 46.9   \\
\hline
\textbf{Blum} & Blum's variant of  & \cite{blum1997empirical} & Multiplicative parameters  & 53.1  \\
& weighted majority & & $\beta=0.5$, $\gamma=1.5$ &  \\
\hline
\textbf{ORL-CF} & Online Relevance Learning  & Our  & $\delta = 0.1$, $\rho=4$, $L=1$  & 0.7  \\
& with Controlled Feedback $D=3$ & work &  &    \\
\hline
\textbf{CON-S} & Contextual Learning with a Single Type    & '' & Same as \textbf{ORL-CF}   & 3.75  \\
\hline
\end{tabular}
}
%\vspace{-0.1in}
\caption{Error percentages of ORL-CF, CON-S and ensemble learning methods.}
%\vspace{-0.3in}
\label{tab:ourbest}
\end{table*}




\comment{Since we only consider single dimensional context, $d=1$. However, due to the bursty, non-stochastic nature of the network security data we cannot find a value $\alpha$ for which Assumption \ref{ass:lipschitz2} is true. Nevertheless, we consider two cases, Z1 and Z2, given in Table \ref{tab:par_setup}, for CoS and DCZA parameter values.
%
In Z2, the parameters for CoS and DCZA are selected according to Theorems 1 and 2 in \cite{cem2013deccontext}, assuming $\alpha=1$. 
%
In Z1, the parameter values are selected in a way that will reduce the number of explorations and trainings. However, the regret bounds for Theorems 1 and 2 in \cite{cem2013deccontext} may not hold for these values in general. 
}




\comment{
In our simulations we consider the performance of learner 1. Table \ref{tab:sim_results} shows under each simulation and parameter setup the percentage of errors made by CoS and DCZA and the percentage of time steps spent in training and exploration phases for learner 1. We compare the performance of DCZA and CoS with AdaBoost, sliding window AdaBoost (SWA), and CoS with no context (but still decentralized different from a standard bandit algorithm) whose error rates are also given in Table \ref{tab:error_comp}. AdaBoost and SWA are trained using 20000 consecutive samples from the data set different from the test data. 
%
SWA re-trains itself in an online way using the last $w$ observations, which is called the window length. Both AdaBoost and SWA are ensemble learning methods which require learner 1 to combine the predictions of all the classification functions. Therefore, when implementing these algorithms we assume that learner 1 has access to all classification functions and their predictions, whereas when using our algorithms we assume that learner 1 only has access to its own classification functions and other learners but not their classification functions. Moreover, learner 1 is limited to use a single prediction in CoS and DCZA. This may be the case in a real system when the computational capability of local learners are limited and the communication costs are high.

First, we consider the case when the parameter values are as given in Z1. We observe that when the context is the previous label, CoS and DCZA perform better than AdaBoost and SWA for both S1 and S2. This result shows that although CoS and DCZA only use the prediction of a single classification function, by exploiting the context information they can perform better than ensemble learning approaches which combine the predictions of all classification functions. We see that the error percentage is smallest for CoS and DCZA when the context is the previous label.
% 
This is due to the bursty nature of the attacks.
%
The exploration percentage for the case when context is the previous label is larger for DCZA than CoS. 
As we discussed in Section \ref{sec:reduction}, the number of explorations of DCZA can be reduced by utilizing the observations from the old hypercube to learn about the accuracy of the arms in a newly activated hypercube. When the context is the feature of the data or the time, for S1, CoS and DCZA perform better than AdaBoost while SWA with window length $w=100$ can be slightly better than CoS and DCZA. But again, this difference is not due to the fact that CoS and DCZA makes too many errors. It is because of the fact that CoS and DCZA explores and trains other classification functions and learners. 
%
AdaBoost and SWA does not require these phases. But they require communication of predictions of all classification functions and communication of all local learners with each other at each time step. Moreover, SWA re-trains itself by using the predictions and labels in its time window, which makes it computationally inefficient.
%
Another observation is that using the feature as context is not very efficient when there are no good classifiers (S2). However, the error percentages of CoS and DCZA ($39\%$ and $38\%$ respectively) are still lower than the error percentage of the best classifier in S2 which is $47\%$. Moreover, CoS and DCZA performs better than CoS with no context for all scenarios with parameter values given by Z1. 
%
We observe that both CoS and DCZA performs poorly when the set of parameters is given by Z2. This is due to the fact that the percentage of training and exploration phases is too large for Z2, thus these algorithms cannot exploit the information they gathered efficiently. Another important reason for the poor performance is the short time horizon. As the time horizon grows, we expect the exploration and training rates to decrease, and the exploitation rate to increase which will improve the performance. 

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.3em}
\begin{tabular}{|l|c|c|}
\hline
(Parameters) Algorithm & (S1) Error $\%$  & (S2) Error $\%$ \\
\hline
(Z1) CoS (previous label as context) & 0.7 & 0.9  \\
\hline
(Z1) DCZA (previous label as context) & 1.4 & 1.9  \\
\hline
AdaBoost & 4.8 & 53  \\
\hline
($w=100$) SWA  & 2.4 & 2.7 \\
\hline
($w=1000$) SWA  & 11 & 11  \\
\hline
(Z1) CoS (no-context) & 5.2 & 49.8  \\
\hline 
\end{tabular}
}
\add{\vspace{-0.05in}}
\caption{Comparison of error percentages of CoS, DCZA, AdaBoost, SWA and CoS with no context.}
\label{tab:error_comp}
\vspace{-0.2in}
%\vspace{-0.4in}
\end{table}

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.3em}
\begin{tabular}{|l|c|c|c|}
\hline
(Setting) & Error $\%$ & Training $\%$ & Exploration $\%$  \\
Algorithm  & context=A1,A2,A3 & context=A1,A2,A3 & context=A1,A2,A3 \\
\hline
(Z1,S1) CoS & 0.7, 4.6, 4.8 & 0.3, 3, 2.8 & 1.4, 6.3, 8.5 \\
\hline
(Z1,S1) DCZA & 1.4, 3.5, 3.2 & 0.4, 1.3, 0.9 & 4, 5.9, 7 \\
\hline
(Z1,S2) CoS & 0.9, 39, 10 & 0.3, 3, 2.8 & 1.5, 6.5, 8.6 \\
\hline
(Z1,S2) DCZA & 1.9, 38, 4.8 & 0.4, 1.3, 1 & 4, 6, 7 \\
\hline
(Z2,S1) CoS & 16, 14, 41 & 8.5, 16, 79 & 55 27 20\\
\hline
(Z2,S1) DCZA & 31, 29, 29 & 33 19 87 & 66 66 12 \\
\hline 
\end{tabular}
}
\add{\vspace{-0.05in}}
\caption{Error, training and exploration percentages of CoS and DCZA under different simulation and parameter settings. (A1) context as the previous label, (A2) context as srcbytes feature, (A3) context as time.}
\label{tab:sim_results}
%\vspace{-0.4in}
\vspace{-0.2in}
\end{table}

\newc{The results in Table \ref{tab:sim_results} are derived for the case when all learners receive the same instance and observe the same label at each time step. Therefore they correspond to the {\em best-case correlation} given in Definition \ref{defn:context}. Moreover, when the context is time, we have {\em worst-case} arrival (as in \textbf{C2}), while when the context is the previous label, arrivals are similar to the {\em best-case arrival} process (as in \textbf{C4}), where instead of a single hypercube of level $\lceil(\log_2 T)/p\rceil +1$, arrivals happen to two different level $\lceil(\log_2 T)/p\rceil +1$ hypercubes one containing $x=0$ and the other one containing $x=1$. 
%
We also run simulations for the worst-case correlation (\textbf{C1} or \textbf{C3}) for CoS (results for DCZA will be similar) for three different contexts A1, A2 and A3. From the results given in Table \ref{tab:sim_results2}, we observe that the exploration and training percentages increases for the worst-case correlation between the learners, which also causes an increase in the error percentages. 
}

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.3em}
\begin{tabular}{|l|c|c|c|}
\hline
(Setting) & Error $\%$ & Training $\%$ & Exploration $\%$  \\
Algorithm & context=A1,A2,A3 & context=A1,A2,A3 & context=A1,A2,A3 \\
\hline
(Z1,S1) CoS & 1.8, 4.1, 6.7 & 2, 9.2, 10.3 & 1.4, 3.6, 8.5 \\
\hline
(Z1,S2) CoS & 24.6, 44.3, 31.3 & 2, 9.2, 10.3 & 1.4, 3.6, 8.5  \\
\hline
\end{tabular}
}
\caption{Error, training and exploration percentages of CoS for  worst-case correlation between the learners for three different context types.}
\label{tab:sim_results2}
\vspace{-0.2in}
%\vspace{-0.4in}
\end{table}

\vspace{-0.1in}
\subsection{Simulation Results for Extensions on CoS and DCZA}

\newc{Firstly, we simulate the ensemble learner given in Section \ref{sec:ensemble} for CoS (called {\em ensemble CoS}), with $d_k=0$ for $k \in {\cal K}_i$, $i \in {\cal M}$. We take time as the context, and consider two different weight update rules. In the {\em context-independent} update rule, weights $w_i(1)$ for each learner is initially set to $1/4$, and $\boldsymbol{w}(t) = (w_1(t),\ldots, w_4(t))$ is updated based on the stochastic gradient descent rule given in Algorithm 2 of \cite{yu2013fast}, with coefficient $1/\alpha$ instead of $1/(\alpha*t)$ to capture the non-stationarity of the incoming data stream where $\alpha=100$. In the {\em context-dependent} update rule, weights for each learner in each set in the partition ${\cal P}_T$ is updated independently from the weights in the other sets based on the same stochastic gradient descent rule.
%
Total error and exploitation error percentages of ensemble CoS is given in Table \ref{tab:weights} for cases S1 and S2. Comparing Tables \ref{tab:sim_results} and \ref{tab:weights}, we see that when the weight update rule is context-independent, there is $21\%$ and $51\%$ improvement in the error of ensemble CoS compared to CoS for cases S1 and S2 respectively. However, when the weight update rule is context dependent, ensemble CoS performs worse than CoS. This is due to the fact that the convergence rate being smaller for context-dependent weights since weights for each $P_l \in {\cal P}_T$ are updated independently. In Table \ref{tab:weights}, we also give the percentage of prediction errors made at the time slots in which all learners are simultaneously in the exploitation phase of CoS. The difference between total error percentage and exploitation error percentage gives the percentage of errors made in exploration steps.
%
\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.3em}
\begin{tabular}{|l|c|c|}
\hline
ensemble CoS & context-dependent weights & context-indep weights \\
Parameters: Z1 & S1, S2 & S1, S2 \\
\hline
total error $\%$ & 5.9, 10.2 & 3.8, 4.94  \\
\hline
exploitation error $\%$ & 2.9, 6.8 & 1.76, 2.17  \\
\hline
\end{tabular}
}
\caption{Total error percentage, and error percentage of the errors made in exploitation steps for CoS with ensemble learner.}
\label{tab:weights}
%\vspace{-0.4in}
\vspace{-0.2in}
\end{table}
%
}
%
\comment{
In Figure \ref{fig:CoS_res} and \ref{fig:DCZA_res}, the number of classification errors is given as a function of time for CoS and DCZA, respectively for S1 and Z1, for all three different context information. The error function is {\em spike-shaped} because of the training phases that happens when a change in the context occurs. Note that when the context is previous label or {\em srcbytes}, the spikes follow the changes in the data, while when the context is time, the spikes are uniformly distributed. 

\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{CoS_res}
\caption{Number of errors made by CoS as a function of time.} 
\label{fig:CoS_res}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{DCZA_res}
\caption{Number of errors made by DCZA as a function of time.} 
\label{fig:DCZA_res}
\end{center}
\end{figure}
}

Secondly, we simulate both CoS and DCZA for the case when the label is not always observed. Our results are given in Table \ref{tab:errorperc} for learner 1 when there are 4 learners. As the probability of observing the label, i.e., $p_r$, decreases, the error percentage of both CoS and DCZA grows. This is due to the fact that more time steps are spent in exploration and training phases to ensure that the estimates of the rewards of arms in ${\cal K}_i$ are accurate enough. 

\comment{
\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
Learner & 1 &2 &3 & 4\\
\hline
Classification  & Naive Bayes,  &Multilayer Perceptron, & RBF Network, & Random Tree,  \\
Function   & Logistic & Voted Perceptron &J48 & Random Forest\\
\hline
 Error  & 42.9,  & 33,  & 43, & 27.5,  \\
percentage & 42.9 & 42.9 &  42.9 & 22\\
\hline
\end{tabular}
}
\add{\vspace{-0.1in}}
\caption{Error percentages of the base classification functions for synthetic data}
\vspace{-0.25in}
\label{tab:basesynt}
\end{table}
}

\comment{
\begin{figure}
\begin{center}
\includegraphics[width=0.8\columnwidth]{error_CoS}
\caption{Error percentage as a function of the probability of observing the label for the instance.} 
\label{fig:somelabel}
\end{center}
\end{figure}
}

Thirdly, in Table \ref{tab:nlearn}, error percentages of CoS and DCZA for learner 1 are given as functions of the number of learners present in the system. Comparing Tables \ref{tab:sim_setup} and \ref{tab:nlearn}, we see that adding a learner whose classification functions are worse than the classification functions of the current learners increases the error percentage due to the increase in the number of training and exploration steps, while adding a learner whose classification functions are better than the best classification function of the current learners decreases the error percentage.

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
(Setting) Algorithm /$p_r$ & 1 & 0.5 & 0.1 & 0.01 \\
\hline
(Z1,S2) CoS (context is time) error $\%$ & 10 & 13.9 & 36.4 & 47.1 \\
\hline
(Z1,S2) DCZA (context is time) error $\%$ & 4.8 & 4.8 & 16.3 & 56.6 \\
\hline
\end{tabular}
}
\caption{Error percentages of CoS and DCZA as a function of $p_r$ (probability of receiving the label at each time slot) when context is time.}
\vspace{-0.2in}
\label{tab:errorperc}
\end{table}


\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
$\#$ of learners & 1 & 2 & 3 & 4 \\
\hline
CoS error $\%$ & 49.8 & 49.7 & 50.2 & 22.3 \\
\hline
DCZA error $\%$ & 49.8 & 49.8 & 49.8 & 22.7 \\
\hline
\end{tabular}
}
\caption{Error percentages of CoS and DCZA for learner 1, as a function of the number of learners present in the system.}
\vspace{-0.2in}
\label{tab:nlearn}
\end{table}


Fourthly, in Table \ref{tab:callcost}, we write the error percentages and the percentage of times each arm in ${\cal K}_i$ is chosen by learner $1$ as a function of the cost of calling other learners for CoS. We let $d_{1_j} = d$ for all $1_j \in {\cal M}_{-1}$. Since the goal of the learner is to maximize the expected accuracy minus cost, we see that learner 1 selects its own classification functions more often as the cost $d$ is increased. However, this results in higher error percentage since classification functions of learner 1 are suboptimal. 

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
d & error $\%$ & training $\%$  & selection (except training/exploration) $\%$  \\
& & of learners 2,3,4 & of learners 1,2,3,4  \\ 
\hline
0 & 0.9 & 0.27, 0.23, 0.16 & 52.9, 47, 0.1, 0\\
\hline
0.5 & 1 & 0.27, 0.23, 0.16 & 53, 47, 0, 0 \\
\hline
0.7 & 23.7 &0.27, 0.23, 0.16 & 100, 0, 0, 0\\
\hline
\end{tabular}
}
\caption{Error and arm selection percentages as a function of calling cost}
\vspace{-0.25in}
\label{tab:callcost}
\end{table}

Finally, in Table \ref{tab:onlycontext}, we give the error percentage of learner 1 using CoS with parameter values Z1, when learner 1 only sends its context information to other learners but not its data. When called by learner 1, other learners do not predict based on their classification functions but they choose the prediction that has the highest percentage of being correct so far at the hypercube that the context of learner 1 belongs.
%
From these results we see that for S1 (two good classification functions), the error percentage of learner 1 is slightly higher than the error percentage when it sends also its data for contexts A1 and A3, while its error percentage is better for context A2. However, for S2 (no good classification functions), sending only context information produces very high error rates for all types of contexts. This suggests correlation of the context with the label and data is not enough to have low regret when only context information is sent. There should be classification functions which have low error rates.
%
Similar results hold for DCZA as well when only context information is sent between the learners. 

\begin{table}[t]
\centering
{\fontsize{8}{6}\selectfont
\setlength{\tabcolsep}{.1em}
\begin{tabular}{|l|c|c|c|c|}
\hline
(Setting) Algorithm & previous label (A1) & srcbytes (A2) & time   \\
& is context & is context & is context \\
\hline
(Z1,S1) CoS error $\%$ & 2.68 & 3.64 & 6.43  \\
\hline
(Z1,S2) CoS error $\%$ & 23.8 & 42.6 & 29 \\
\hline
\end{tabular}
}
\caption{Error percentages of CoS for learner 1, when learner 1 only sends its context information to the other learners.}
\vspace{-0.3in}
\label{tab:onlycontext}
\end{table}
}









==> futurework.tex <==
\section{Future Work} \label{sec:future}
